Stochastic Adaptive Neural Architecture Search for Keyword Spotting

The problem of keyword spotting i.e. identifying keywords in a real-time audio stream is mainly solved by applying a neural network over successive sliding windows. Due to the difficulty of the task, baseline models are usually large, resulting in a high computational cost and energy consumption level. We propose a new method called SANAS (Stochastic Adaptive Neural Architecture Search) which is able to adapt the architecture of the neural network on-the-fly at inference time such that small architectures will be used when the stream is easy to process (silence, low noise, ...) and bigger networks will be used when the task becomes more difficult. We show that this adaptive model can be learned end-to-end by optimizing a trade-off between the prediction performance and the average computational cost per unit of time. Experiments on the Speech Commands dataset show that this approach leads to a high recognition level while being much faster (and/or energy saving) than classical approaches where the network architecture is static.

==> results/big_table_6row.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small{
\begin{tabular}{|c|ccccc|}
\hline
\textbf{Model}                    & \textbf{Match} & \textbf{Correct} & \textbf{Wrong} & \textbf{FA} & \textbf{FLOPs} \\ \hline
\textit{\textbf{cnn-trad-fpool3}} & 81.7\%         & 72.8\%           & 8.9\%          & 0.0\%       & 124.6M       \\ \hline
\multirow{14}{*}{\textbf{SANAS}}  & 0.0\%          & 0.0\%            & 0.0\%          & 0.0\%       & 0.0         \\
                                  & 61.2\%         & 53.8\%           & 7.3\%          & 0.7\%       & 519.2K       \\
                                  & 48.0\%         & 38.3\%           & 9.7\%          & 0.4\%       & 526.4K       \\
                                  & 62.0\%         & 57.3\%           & 4.8\%          & 0.1\%       & 22.9M        \\
                                  & 86.5\%         & 80.7\%           & 5.8\%          & 0.3\%       & 37.7M        \\
                                  & 85.0\%         & 79.6\%           & 5.4\%          & 0.2\%       & 38.6M        \\
                                  & 83.7\%         & 79.3\%           & 4.4\%          & 0.3\%       & 44.2M        \\
                                  & 83.5\%         & 78.2\%           & 5.3\%          & 0.0\%       & 44.8M        \\
                                  & 85.8\%         & 80.6\%           & 5.3\%          & 0.2\%       & 45.2M        \\
                                  & 86.3\%         & 80.6\%           & 5.7\%          & 0.2\%       & 48.8M        \\
                                  & 84.1\%         & 78.0\%           & 6.1\%          & 0.0\%       & 51.4M        \\
                                  & 81.7\%         & 76.4\%           & 5.3\%          & 0.1\%       & 94.0M        \\
                                  & 80.7\%         & 75.6\%           & 5.1\%          & 0.1\%       & 101.9M       \\
                                  & 81.4\%         & 76.3\%           & 5.2\%          & 0.2\%       & 105.4M       \\ \hline
\end{tabular}
}
\caption{Evaluation of models on 1h of audio from \cite{DBLP:Warden_speech_commands} containing words roughly every 3 seconds with different background noises. We use the label post processing and the streaming metrics proposed in \cite{DBLP:Warden_speech_commands} to avoid the inconvenient illustrated in Figure \ref{fig:data}, repeated detection and noisy detections. Matched \% corresponds to the portion of words detected, either correctly (Correct \%) or incorrectly (Wrong \%). False Alarms (FA) are omitted because always $<0.3\%$}
\label{tab:streaming}
\end{table}

==> results/cnn-trad-fpool3.tex <==
\begin{table}[]
\begin{tabular}{|l|ll|}
\hline
Model           & Test Accuracy & Average FLOPs \\ \hline
\hline
cnn-trad-fpool3 &       -        &        -       \\ \hline
Baseline min    &       -        &        -       \\ \hline
Baseline max    &       -        &       -     \\ \hline
AdaptNet (ours) &       -        &       -        \\ \hline
\end{tabular}
\end{table}

==> results/new_stream_eval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

\begin{tabular}{|c||cccc|}
\hline
Model                                        & Matched         & Correct         & Wrong          & FLOPs           \\ \hline\hline
%Reference \cite{DBLP:Warden_speech_commands} & 50.3\%          & 47.2\%          & \textbf{3.1\%} &                \\ \hline
\textit{cnn-trad-fpool3}                     & 81.7\%          & 72.8\%          & 8.9\%          & 124.6M         \\ \hline
\multirow{4}{*}{\textbf{SANAS}}              & \textbf{84.1\%} & \textbf{78.0\%} & 6.1\%          & 51.4M          \\
                                             & 79.5\%          & 75\%            & \textbf{4.5}\%          & 47.9M          \\
                                             & 77.8\%          & 72.1\%          & 5.7\%          & 36.5M \\
                                             
                                             & 61.3\%          & 53.3   \%          & 8.0 \%          & \textbf{519K} \\\hline
\end{tabular}

\caption{Evaluation of models on 1h of audio from \cite{DBLP:Warden_speech_commands} containing words roughly every 3 seconds with different background noises. We use the label post processing and the streaming metrics proposed in \cite{DBLP:Warden_speech_commands} to avoid the inconvenient illustrated in Figure \ref{fig:data}, repeated detection and noisy detections. Matched \% corresponds to the portion of words detected, either correctly (Correct \%) or incorrectly (Wrong \%). False Alarms (FA) are omitted because always $<0.3\%$}
\label{tab:streaming}
\end{table}

==> results/new_stream_eval_2.tex <==
\begin{table}[]
\begin{tabular}{|cccccc|}
\hline
\textbf{Match}    & \textbf{Correct}   & \textbf{Wrong}  & \textbf{FA}      & \textbf{FLOPs}      & \textbf{Acc}     \\ \hline \hline
\multicolumn{6}{|c|}{\textbf{\textit{cnn-trad-fpool3}}} \\ \hline
81.7\%   & 72.8\%    & 8.9\%   & 0.0\%   & 124.6M   & 70.4\%  \\ \hline \hline
\multicolumn{6}{|c|}{\textbf{\textit{cnn-trad-fpool3} + shortcuts}}                              \\ \hline
57.1\%         & 52.3\%           & 4.8\%          & 0.3\%       & 137.3M       & 72.7\%       \\ \hline \hline
\multicolumn{6}{|c|}{\textbf{SANAS}}           \\ \hline
0.0\%    & 0.0\%     & 0.0\%   & 0.0\%   & 0.0     & 66.6\%  \\
61.2\%   & 53.8\%    & 7.3\%   & 0.7\%   & 519.2K   & 68.7\%  \\
62.0\%   & 57.3\%    & 4.8\%   & 0.1\%   & 22.9M    & 64.5\%  \\
77.7\%   & 73.2\%    & 4.5\%   & 0.2\%   & 37.5M    & 65.2\%  \\
78.2\%   & 73.4\%    & 4.8\%   & 0.2\%   & 37.6M    & 68.0\%  \\
85.0\%   & 79.6\%    & 5.4\%   & 0.2\%   & 38.6M    & 72.0\%  \\
80.1\%   & 75.6\%    & 4.5\%   & 0.1\%   & 39.6M    & 70.0\%  \\
83.7\%   & 79.3\%    & 4.4\%   & 0.3\%   & 44.2M    & 70.7\%  \\
83.5\%   & 78.2\%    & 5.3\%   & 0.0\%   & 44.8M    & 70.6\%  \\
85.8\%   & 80.6\%    & 5.3\%   & 0.2\%   & 45.2M    & 74.1\%  \\
86.3\%   & 80.6\%    & 5.7\%   & 0.2\%   & 48.8M    & 72.0\%  \\
84.1\%   & 78.0\%    & 6.1\%   & 0.0\%   & 51.4M    & 72.0\%  \\
81.7\%   & 76.4\%    & 5.3\%   & 0.1\%   & 94.0M    & 75.2\%  \\
80.7\%   & 75.6\%    & 5.1\%   & 0.1\%   & 101.9M   & 74.8\%  \\
81.4\%   & 76.3\%    & 5.2\%   & 0.2\%   & 105.4M   & 73.9\%  \\ \hline
\end{tabular}




\caption{Evaluation of models on 1h of audio from \cite{DBLP:Warden_speech_commands} containing words roughly every 3 seconds with different background noises. We use the label post processing and the streaming metrics proposed in \cite{DBLP:Warden_speech_commands} to avoid the inconvenient illustrated in Figure \ref{fig:data}, repeated detection and noisy detections. Matched \% corresponds to the portion of words detected, either correctly (Correct \%) or incorrectly (Wrong \%). }
\label{tab:streaming}
\end{table}

==> results/stream_kwscnn.tex <==
\begin{table}[]
\begin{tabular}{|ccc|}
\hline
Model                                                   & \begin{tabular}[c]{@{}c@{}}Classification\\  error (\%)\end{tabular} & Average FLOPs \\ \hline
cnn-trad-fpool3 \cite{DBLP:conf/interspeech/SainathP15} & 29.6                                                            & 124.6M        \\
cnn-trad-fpool3 + SANAS                                 & 18.1                                                            & 40.0M         \\
cnn-trad-fpool3 + SANAS                                 & 17.7                                                            & 44.9M         \\ \hline
ResNet \cite{DBLP:conf/icassp/TangL18}                  & 22.7                                                            & 35.7M         \\
ResNet + SANAS                                          & 25.2                                                            & 6M            \\
ResNet + SANAS                                          & 24.8                                                            & 7.7M          \\ \hline
\end{tabular}
\caption{\textcolor{red}{Preliminary results..... New experiments have been launched since the previous implementation had some bugs...}Evaluation of models on 1h of audio containing words roughly every 3 seconds, with different background noises added at variable SNR ratios. We use the file created in \cite{DBLP:Warden_speech_commands} as a common benchmark.}
\label{tab:streaming}
\end{table}
